Parallel Nearest Neighbors in Low Dimensions with Batch Updates

We present a set of parallel algorithms for computing exact k-nearest neighbors in low dimensions. Many k-nearest neighbor algorithms use either a kd-tree or the Morton ordering of the point set; our algorithms combine these approaches using a data structure we call the \textit{zd-tree}. We show that this combination is both theoretically efficient under common assumptions, and fast in practice. For point sets of size $n$ with bounded expansion constant and bounded ratio, the zd-tree can be built in $O(n)$ work with $O(n^{\epsilon})$ span for constant $\epsilon<1$, and searching for the $k$-nearest neighbors of a point takes expected $O(k\log k)$ time. We benchmark our k-nearest neighbor algorithms against existing parallel k-nearest neighbor algorithms, showing that our implementations are generally faster than the state of the art as well as achieving 75x speedup on 144 hyperthreads. Furthermore, the zd-tree supports parallel batch-dynamic insertions and deletions; to our knowledge, it is the first k-nearest neighbor data structure to support such updates. On point sets with bounded expansion constant and bounded ratio, a batch-dynamic update of size $k$ requires $O(k \log n/k)$ work with $O(k^{\epsilon} + \text{polylog}(n))$ span.

==> Algorithms/algo-batchdyn.tex <==
\begin{algorithm2e}[t]
	\caption{batch\_insert($T, P, B)$\protect\\
The batch-dynamic insertion algorithm. The function morton\_sort refers to sorting according to the Morton ordering of the point set.}
	\label{algo: batchdyn}\small
	\SetAlgoLined
	\KwIn{A pointer to the root of a kd-tree $T$, a list of points $P$ to insert, and a bounding box $B$}
	\KwOut{A pointer to the root of the kd-tree containing all points in the original tree, plus the points in $P$}
	\uIf{$P$ not contained in $B$} {\KwRet{error()}} 
	morton\_sort($P$) \;
	batch\_insert\_rec(T, P) \;
	\KwRet{T}
	\vspace{0.5em}
\end{algorithm2e}

==> Algorithms/algo-epsbox.tex <==
\begin{algorithm2e}[t!]
	\caption{within\_epsilon\_box($T, p, \epsilon)$\protect
}
	\label{algo: withinepsbox}\small
	\SetAlgoLined
	\KwIn{A pointer to the vertex of a kd-tree $T$, a point $p$, and a double $\epsilon$}
	\KwOut{Bool}
	$B \leftarrow T$.Box()\;
	result $\leftarrow$ True\;
	$d \leftarrow$ dimension($p$)\;
	\For{$i\leftarrow 1$ \KwTo $d$}{
		first $\leftarrow B$.first[$i$]$-\epsilon \leq p$[i]\;
		second $\leftarrow B$.second[$i$]$+\epsilon \geq p$[i]\;
		result = result \&\& first \&\& second \;
	}
	\KwRet{result}
	\vspace{0.5em}
\end{algorithm2e}

==> Algorithms/algo-nnsearch.tex <==
\begin{algorithm2e}[t]
	\caption{k\_nearest($T, p, k)$\protect\\
The full nearest neighbor search algorithm.}
	\label{algo: nnsearch}\small
	\SetAlgoLined
	\KwIn{A pointer to the root of a kd-tree $T$ and a point $p$}
	\KwOut{A vector $v$ containing the k-nearest neighbors of $p$}
	$v \leftarrow $ vector in $k$ dimensions \;
	\For{$i\leftarrow 1$ \KwTo $k$}{
		$v[i] \leftarrow \infty$\;
	}
	$L$ = find\_leaf($T$, $p$)\;
	search\_up($L, p$) \;
	\KwRet{v}


	\vspace{0.5em}
\end{algorithm2e}

==> figure-STANNvParlay.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=.8\columnwidth]{figures/3DSTANNvParlayFig}
\end{center}\vspace{-1.5em}
\caption{\small Performance of the original Connor and Kumar k-nearest neighbors implementation using OpenMP compared with the modified version of their code using ParlayLib. Tests were performed using a 3D random dataset of 10 million points.}
\label{fig: STANNvParlay}
\vspace{-1em}
\end{figure}

==> figure-gridpic.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=.7\columnwidth]{figures/GridPic} \\
\end{center}\vspace{-1.5em}
\caption{\small A graphic illustrating a box situated inside the largest possible quad-tree box. Note that the $2^d$ boxes that are formed by the cut of the blue box are each contained in a quad-tree box of at most the side length of the blue box.}
\label{fig: gridpic}
\end{figure}

==> figure-gridsquares.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=.7\columnwidth]{figures/GridSquares} \\
\end{center}\vspace{-1.5em}
\caption{\small A graphic showing the quadtree box of radius $r$ that contains the initial approximation of nearest neighbors of point $p$. The box is shown in red, while the quadtree boxes which may contain neighbors of $p$ are shown in black.}
\label{fig: gridsquares}
\end{figure}

==> figure-leafsearch.tex <==
\begin{figure*}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=.66\columnwidth]{figures/Grid}
  \includegraphics[width=.66\columnwidth]{figures/Tree}
  \includegraphics[width=.66\columnwidth]{figures/Tree2}
\end{center}\vspace{-1.5em}
\caption{\small To the far left, a collection of points, with the point we desire to find the nearest neighbor of marked in green. In the middle and to the far right, a quadtree where each leaf represents one square of the grid. In the left quadtree, the nodes searched when searching for the target point's nearest neighbor when searching from the root; on the right, the nodes searched when searching from the leaf containing the query point.}
\label{fig: rootsearch}
\vspace{-1em}
\end{figure*}

==> figure-nodechart.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
	\tabcolsep=0.09cm
	\begin{tabular}{|c|c|c|c|c|} 
	\hline
	\begin{tabular}{c}
		Search \\
		From?
	\end{tabular} & Dataset & \begin{tabular}{c}
	Average \\ Nodes \\
	Searched
\end{tabular} & \begin{tabular}{c}
Maximum \\ Nodes \\
Searched
\end{tabular} & \begin{tabular}{c}
Tree \\ Depth
\end{tabular} \\
	\hline
	Root & \begin{tabular}{c}
		2DinCube \\
		2Dkuzmin \\
		3DinCube \\
		3DonSphere \\
		3Dplummer \\
	\end{tabular} &
	 \begin{tabular}{c}
		42.48 \\
		117.1 \\
		52.1 \\
		100.9 \\
		359.9 \\
	\end{tabular}
	& \begin{tabular}{c}
		145 \\
		1516859 \\
		263 \\
		132 \\
		1520401 \\
	\end{tabular} & \begin{tabular}{c}
	20 \\
	61 \\
	20 \\
	28 \\
	54 \\
\end{tabular} \\
	\hline
	Leaf & 	\begin{tabular}{c}
		2DinCube \\
		2Dkuzmin \\
		3DinCube \\
		3DonSphere \\
		3Dplummer \\
	\end{tabular} &
	\begin{tabular}{c}
		4.578 \\
		4.764 \\
		17.51 \\
		6.54 \\
		52.42 \\
	\end{tabular}
	& \begin{tabular}{c}
		125 \\
		1516857 \\
		242 \\
		131 \\
		1520399 \\
	\end{tabular} & - \\
	\hline
\end{tabular}
\end{center}\vspace{-1.0em}
\caption{\small Searching for nearest neighbors from the root vs from the leaf is compared for several different datasets. The chart shows both the average number of kd-tree nodes searched per query, and the largest number of nodes searched for any single query.}
\label{fig: visitedchart}
\end{figure}

==> figure-nondynamicdata.tex <==

\begin{figure*}[t]
	\vspace{-.5em}
	\input{figures/2Dvaryingdataset}
	\input{figures/3Dvaryingdataset}
	\input{figures/3Dvaryneighbors}
	\input{figures/3DbyThread}
	\input{figures/3DbyThreadParallel}
	\caption{\small }
	\label{fig: nondynamicdata}
	\vspace{-1em}
\end{figure*}

==> figure-searchimprove.tex <==

\begin{figure}[t]
	\vspace{-.5em}
	\begin{center}
	\begin{tabular}{|c|c|c|}
	\hline
	Method & Average Searched & Max Searched \\
	\hline
	Start from root & \begin{tabular}{c}
		2DinCube\_10M: 42.48 \\
		2Dkuzmin\_10M: 117.1 \\
		3DinCube\_10M: 52.1 \\
		3DonSphere\_10M: 100.9 \\
		3DinCube\_10M: 79.68 \\
		3Dplummer\_10M: 359.9 \\
	\end{tabular}
	& \begin{tabular}{c}
		2DinCube\_10M: 145 \\
		2Dkuzmin\_10M: 1516859 \\
		3DinCube\_10M: 263 \\
		3DonSphere\_10M: 1321 \\
		3DinCube\_10M: 285 \\
		3Dplummer\_10M: 1520401 \\
	\end{tabular} \\
	\hline
	Start from leaf & \begin{tabular}{c}
		2DinCube\_10M: 4.578 \\
		2Dkuzmin\_10M: 4.764 \\
		3DinCube\_10M: 17.51 \\
		3DonSphere\_10M: 6.54 \\
		3DinCube\_10M: 48.58 \\
		3Dplummer\_10M: 52.42 \\
	\end{tabular}
	& \begin{tabular}{c}
		2DinCube\_10M: 125 \\
		2Dkuzmin\_10M: 1516857 \\
		3DinCube\_10M: 242 \\
		3DonSphere\_10M: 131 \\
		3DinCube\_10M: 265 \\
		3Dplummer\_10M: 1520399 \\
	\end{tabular} \\
	\hline
\end{tabular}
	\end{center}\vspace{-1.5em}
	\caption{\small }
	\label{fig: searchimprove}
	\vspace{-1em}
\end{figure}





==> figure-tinybox.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=.7\columnwidth]{figures/dboxes} \\
\end{center}\vspace{-1.5em}
\caption{\small A figure illustrating the setup in Theorem~\ref{thm: treebuild}. Here, the empty boxes represent splits with no points, the light blue boxes represent unbalanced splits, and the dark blue box represents the box containing $p$ after the two splits.}
\label{fig: tinybox}
\end{figure}

==> prelims.tex <==
\section{Preliminaries}\label{sec: prelims}

Here we provide a few preliminaries. 
